Galactic Panspermia

We present an analytic model to estimate the total number of rocky or icy objects that could be captured by planetary systems within the Milky Way galaxy and result in panspermia should they harbor life. We estimate the capture rate of objects ejected from planetary systems over the entire phase space as well as time. Our final expression for the capture rate depends upon the velocity dispersion as well as the characteristic biological survival time and the size of the captured object. We further take into account the number of stars that an interstellar object traverses, as well as the scale height and length of the Milky Way's disk. The likelihood of Galactic panspermia is strongly dependent upon the survival lifetime of the putative organisms as well as the velocity of the transporter. Velocities between $10-100$ km s$^{-1}$ result in the highest probabilities. However, given large enough survival lifetimes, even hypervelocity objects traveling at over 1000 km s$^{-1}$ have a significant chance of capture, thereby increasing the likelihood of panspermia. Thus, we show that panspermia is not exclusively relegated to solar-system sized scales, and the entire Milky Way could potentially be exchanging biotic components across vast distances.

==> journal_abbr.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                                             %
% Common Journal Abbreviations                                                %
%                                                                             %
%   Include using the '\input{journal_abbr}' command in preamble.             %
%                                                                             %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\aap{A\&A} %.......................Astronomy and Astrophysics
\def\aaps{A\&AS} %.....................Astronomy and Astrophysics Supplement Series
\def\aj{AJ} %..........................Astronomical Journal
\def\apj{ApJ} %........................Astrophysical Journal
\def\apjl{ApJL} %......................Astrophysical Journal Letters
\def\apjs{ApJS} %......................Astrophysical Journal Supplement Series
\def\apss{Ap\&SS} %....................Astrophysics and Space Science
\def\araa{ARAA} %......................Annual Reviews of Astronomy and Astrophysics
\def\josa{J.~Opt.~Soc.~Am.} %..........Journal of the Optical Society of America
\def\jpp{J.~Plasma Phys.} %............Journal of Plasma Physics
\def\mnras{MNRAS} %....................Monthly Notices of the Royal Astronomical Society
\def\nat{Nature} %.....................Nature
\def\ptrs{Phil.~Trans.~Roy.~Soc.} %....Philosophical Transactions of the Royal Society
\def\physrep{Phys.~Rep.} %.............Physics Reports
\def\plb{Phys. Lett. B} %..............Physics Letters B
\def\pp{Phys.~Plasma} %................Physical Plasmas
\def\prl{Phys.~Rev.~Lett.} %...........Physical Review Letters
\def\pr{Phys.~Rev.} %..................Physical Review
\def\prd{Phys.~Rev.~D} %...............Physical Review D
\def\pre{Phys.~Rev.~E} %...............Physical Review E
\def\pasj{Publ.~Astron.~Soc.~Japan} %..Publications of the Astronomical Society of Japan
\def\pasp{PASP} %......................Publications of the Astronomical Society of the Pacific
\def\prs{Proc.~Roy.~Soc.} %............Proceedings of the Royal Society
\def\rpp{Rep.~Prog.~Phys.}%............Reports on Progress in Physics
\def\rmp{Rev.~Mod.~Phys.}%.............Reviews of Modern Physics
\def\sci{Science} %....................Science

